Biblioranking fundamental physics

We propose measures of the impact of research that improve on existing ones such as counting of number of papers, citations and $h$-index. Since different papers and different fields have largely different average number of co-authors and of references we replace citations with individual citations, shared among co-authors. Next, we improve on citation counting applying the PageRank algorithm to citations among papers. Being time-ordered, this reduces to a weighted counting of citation descendants that we call PaperRank. Similarly, we compute an AuthorRank applying the PageRank algorithm to citations among authors. These metrics quantify the impact of an author or paper taking into account the impact of those authors that cite it. Finally, we show how self- and circular- citations can be eliminated by defining a closed market of citation-coins. We apply these metrics to the InSpire database that covers fundamental physics, ranking papers, authors, journals, institutes, towns, countries, continents, genders, for all-time and in recent time periods.

==> tabs/Instit2010.tex <==
\begin{tabular}{lc}
  Institution & After 2010 \\  \hline 
\color{red}\bf \color{red}\bf CERN & \color{red}\bf 770\\
\color{magenta}\bf \color{magenta}\bf Princeton, Inst & \color{magenta}\bf 358\\
\color{brown}\bf \color{brown}\bf Perimeter Inst. & \color{brown}\bf 357\\
\bf \bf Fermilab & \bf 328\\
\bf \bf Cambridge U., D & \bf 221\\
\bf \bf Brookhaven & \bf 212\\
\bf \bf DESY & \bf 190\\
\bf \bf Caltech & \bf 187\\
\bf \bf Princeton U. & \bf 178\\
\bf \bf Munich, Max Pla & \bf 178\\
Dubna, JINR & 167\\
Potsdam, Max Pl & 161\\
Imperial Coll., & 159\\
KEK, Tsukuba & 154\\
Tokyo U., IPMU & 154\\
Valencia U., IF & 151\\
Stanford U., Ph & 148\\
SLAC & 148\\
Maryland U. & 134\\
Heidelberg, Max & 133\\
Harvard U. & 132\\
UC, Santa Barba & 128\\
Harvard U., Phy & 126\\
Kyoto U., Yukaw & 123\\
Beijing, Inst.  & 122\\
Washington U.,  & 120\\
SUNY, Stony Bro & 118\\
UC, Berkeley & 116\\
Heidelberg U. & 114\\
MIT & 113\\
Stanford U., IT & 111\\
Durham U., IPPP & 110\\
Munich, Tech. U & 109\\
LBL, Berkeley & 107\\
Moscow, ITEP & 105\\
McGill U. & 105\\
Southampton U. & 104\\
Frankfurt U. & 103\\
Madrid, IFT & 100\\
Saclay, SPhT & 98\\
Orsay, LPT & 98\\
Cracow, INP & 97\\
Tokyo U. & 95\\
Kyoto U. & 95\\
Jefferson Lab & 94\\
Pennsylvania U. & 93\\
MIT, LNS & 93\\
UC, Irvine & 92\\
Ohio State U. & 92\\
Tata Inst. & 89\\
MIT, Cambridge, & 88\\
Humboldt U., Be & 87\\
Zurich U. & 86\\
UCLA & 86\\
Santa Barbara,  & 86\\
Penn State U. & 85\\
Zurich, ETH & 85\\
Weizmann Inst. & 84\\
Bohr Inst. & 83\\
Columbia U. & 82\\
APC, Paris & 81\\
Utrecht U. & 81\\
Florida U. & 81\\
British Columbi & 80\\
SISSA, Trieste & 78\\
Bonn U. & 78\\
Oxford U. & 78\\
INFN, Turin & 77\\
YITP, Stony Bro & 77\\
Beijing, Inst.  & 77\\
Kennesaw State  & 77\\
Marseille, CPT & 76\\
IPhT, Saclay & 76\\
Oxford U., Theo & 74\\
Korea Inst. Adv & 74\\
Warsaw U. & 73\\
Moscow, INR & 73\\
NIKHEF, Amsterd & 73\\
Harish-Chandra  & 73\\
Munich U., ASC & 72
\end{tabular}
